An Empirical Study on the Relationship Between the Number of Coordinated Views and Visual Analysis

Coordinated Multiple views (CMVs) are a visualization technique that simultaneously presents multiple visualizations in separate but linked views. There are many studies that report the advantages (e.g., usefulness for finding hidden relationships) and disadvantages (e.g., cognitive load) of CMVs. But little empirical work exists on the impact of the number of views on visual anlaysis results and processes, which results in uncertainty in the relationship between the view number and visual anlaysis. In this work, we aim at investigating the relationship between the number of coordinated views and users analytic processes and results. To achieve the goal, we implemented a CMV tool for visual anlaysis. We also provided visualization duplication in the tool to help users easily create a desired number of visualization views on-the-fly. We conducted a between-subject study with 44 participants, where we asked participants to solve five analytic problems using the visual tool. Through quantitative and qualitative analysis, we discovered the positive correlation between the number of views and analytic results. We also found that visualization duplication encourages users to create more views and to take various analysis strategies. Based on the results, we provide implications and limitations of our study.

==> 10-Introduction-old.tex <==
\section{Introduction}


Analyzing multidimensional datasets can be challenging due to the difficulty in inspecting entities and groups of entities by many different factors.
A common visualization approach to supporting such analysis is to use \textit{multiple coordinated views} (MCVs)~\cite{North00, Baldonado00} to simultaneously presents multiple visualizations in separate but linked views. 
MCVs provide many benefits for analysis by allowing users to explore trends from different perspectives, to collect and organize multiple relationships, to identify hidden trends, and to obtain insights through a variety of interactions coordinated between multiple views~\cite{Baldonado00, North00, Roberts04}. 

However, the investigation of multidimensional data with multiple views may also introduce difficulty due to its flexibility in the ability to support numerous data views.
Exploratory analysis often benefits from analysts considering multiple paths during open-ended sensemaking~\cite{Pirolli05} and knowledge generation processes~\cite{Sacha14}.
Users often employ branching lines of thought while creating multiple hypotheses for testing and validation.
Keeping track of such branching analyses can be challenging with MCVs due to the number of views and the need to continuously select and adjust chosen attributes for investigation (e.g.,~\cite{Saraiya05,Dunne12,Gotz09}).
To alleviate such issues, many visual analysis tools have started providing \textit{visualization duplication (VD)} as an efficient method for creating a copy of an existing visualization or view.
This way, changes can be made to one of the two views while keeping the other for reference.
A number of commercial tools (e.g., Tableau, Spotfire) support this approach by allowing users to easily copy an existing visualization with one or two clicks. 
Roberts et al.~\cite{Roberts14} discuss numerous benefits to supporting duplication functionality such as copying, cutting, and pasting of pre-existing visualization views to help the user maintain understanding of state and history during analysis. 
Taking duplication a step further, numerous researchers have demonstrated support for branching trails of views to assist showing sequences of logic, operations, and view generation (e.g.,~\cite{Bavoil05,Tobiasz09,Dunne12}).

Although visualization duplication designs hold obvious benefits, less is known about the interaction techniques and interface design options for supporting effective use of duplication functions during visual analysis.
In order to design visualization tools with duplication techniques that can assist users in comparing threads of logic, keeping track of their analysis history during branching analysis, and effectively backtracking or context switching during complex analysis scenarios, it is important to understand how analysts use duplication.
Little empirical research exists on how visualization duplication influences analysis strategies and interaction behaviors. 
Thus, in our research, we aim to better understand analysis processes for users working with MCV tools that allow duplication for real-time data exploration.




We present a study comparing analysis strategies and performances for participants using MCV visualization tools supporting and not supporting visualization duplication. 
In a between-subjects experiment, participants ($n=44$) performed visual data analysis tasks on a multidimensional dataset about automobiles. 
Each participant was assigned to one of two groups: 1) the \textit{Duplication Group} (DG) that had access to tool with visualization duplication, or the 2) \textit{Control Group} (CG), which used an identical version of the tool except without the duplication feature.
Our experiment results indicate that the participants who had access to \tech{} 1) created more views, 2) performed more interactions during visual analysis, 3) completed tasks more accurately, and 4) developed various problem-solving patterns and strategies.
However, no significant results were observed in terms of time spent and participants' confidence levels.
In addition, we observe that participants with the duplication feature showed interesting annotation usage and interaction patterns.



































==> 7-1FrequentInteractionSequences.tex <==

\begin{table}[t]
 \scriptsize
 \begin{center}
   \begin{tabular}{cccc}
     \textbf{Control Group} & \textbf{Interaction Patterns} & \textbf{Experiment Group}\\
   \hline
        2.93 ($\sigma=2.63$) & \begin{tabular}[c]{@{}c@{}}\textbf{Orienting*} \\ 
        Filter-Reconfigure-Filter\end{tabular}  & 5.76 ($\sigma=4.90$)\\ \hline
        12.07 ($\sigma=8.37$)& \begin{tabular}[c]{@{}c@{}}\textbf{Narrowing}\\ Retrieve-Filter-Retrieve\end{tabular}   & 17.35 ($\sigma=16.98$)\\ \hline
        0.21 ($\sigma=0.41$)& \begin{tabular}[c]{@{}c@{}}\textbf{Comparing}\\ Reconfigure-Filter-Reconfigure\\-Filter-Annotation\end{tabular} & 0.45 ($\sigma=0.77$)\\ \hline
        0.57 ($\sigma=0.90$)& \begin{tabular}[c]{@{}c@{}}\textbf{Externalizing 1}\\ Reconfigure-Filter\\-Annotation-Filter\end{tabular}   & 0.76 ($\sigma=0.93$)\\ \hline
        3.21 ($\sigma=3.71$) & \begin{tabular}[c]{@{}c@{}}\textbf{Externalizing 2}\\ Retrieve-Filter-Annotation-Filter\end{tabular}   & 2.93 ($\sigma=3.46$)\\\hline  
   \end{tabular}
  \caption{The average interaction pattern numbers identified from SPAM~\cite{Ayres02}. DG participants performed Orienting more often than those in CG.}
  \label{table_pattern_count_spam}
   \end{center}
\end{table}

\begin{table}[t]
 \scriptsize
 \begin{center}
   \begin{tabular}{@{}ccccc@{}}
     & \textbf{Orienting} & \textbf{Narrowing} & \textbf{Comparing} & \textbf{Externalizing} \\
   \hline
     \textbf{Observation}  & \begin{tabular}[c]{@{}c@{}}$r=0.66$ \\ 
        \textbf{($p<0.001$)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$r=0.68$ \\ 
        \textbf{($p<0.001$)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$r=0.87$ \\ 
        \textbf{($p<0.001$)}\end{tabular} &  \begin{tabular}[c]{@{}c@{}}$r=0.55$  \\ 
        \textbf{($p=0.02$)}\end{tabular} \\
   \hline
     \textbf{Hypothesis} & \begin{tabular}[c]{@{}c@{}}$r=0.80$ \\ 
        \textbf{($p=0.03$)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$r=0.45$ \\ 
        \textbf{($p<0.001$)}\end{tabular}& \begin{tabular}[c]{@{}c@{}}$r=0.88$ \\ 
        \textbf{($p=0.01$)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$r=0.38$ \\ 
        (n.s)\end{tabular} \\
   \hline
     \textbf{Question} & \begin{tabular}[c]{@{}c@{}}$r=0.67$ \\ 
        \textbf{($p<0.001$)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$r=0.49$  \\ 
        \textbf{($p=0.01$)}\end{tabular}& \begin{tabular}[c]{@{}c@{}}$r=0.96$ \\ 
        \textbf{($p<0.001$)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$r=0.45$  \\ 
        \textbf{($p=0.02$)}\end{tabular} \\
   \hline
     \textbf{Goal} & \begin{tabular}[c]{@{}c@{}} $r=0.16$ \\ 
        (n.s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$r=0.19$  \\ 
        (n.s)\end{tabular}& \begin{tabular}[c]{@{}c@{}}$r=0.11$ \\ 
        (n.s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$r=0.27$  \\ 
        (n.s)\end{tabular} \\
   \hline
     \textbf{Comment} & \begin{tabular}[c]{@{}c@{}} $r=0.44$\\ 
        \textbf{($p=0.03$)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$r=0.63$  \\ 
        \textbf{($p<0.001$)}\end{tabular}& \begin{tabular}[c]{@{}c@{}}$r=0.48$ \\ 
        \textbf{($p=0.01$)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$r=0.04$  \\ 
        (n.s)\end{tabular} \\
   \hline
   \end{tabular}
    \caption{Computed correlations between interaction patterns and insight types. Note that ``Comparing” has a very strong correlation with Observation, Hypothesis, and Questions. P values are shown for significant effects, and ``ns'' indicates \textit{no significance}.}
     \label{tab_correlation}
 \end{center}
\end{table}



\subsection{Frequent Interaction Sequences}\label{sec_activities}
We derived four interaction sequences that were frequently performed during the visual analysis using SPAM and Yi et al.'s interaction taxonomy~\cite{Yi07}. We define the interaction sequences as four analytical activities as presented below:
\begin{itemize}
\item \textbf{Orienting}:
(\textit{Filter-Reconfigure-Filter}) Participants filter (e.g., PCP range filtering) the data, confirm a new aspect of the data by reconfiguring (e.g., PCP axis moving), and then filter again.
\item \textbf{Narrowing}: (\textit{Retrieve-Filter-Retrieve}) Participants look at values in the table, filter for specific data, and read the new values in the table.
\item \textbf{Comparing}:
(\textit{Reconfigure-Filter-Reconfigure-Filter-Annotate}) Participants see data and ask new data again for comparison before they write a conclusion.
\item \textbf{Externalizing}:
(\textit{Reconfigure-Filter-Annotate-Filter};  \textit{Retrieve-Filter-Annotate-Filter})
Participants see a new aspect of the data, ask for specific data, make annotations for externalizing insights, and then ask other data for further investigation. 
\end{itemize}

After defining the activities, we observed that two different interaction sequences can represent Externalizing, as shown in Table~\ref{table_pattern_count_spam}.  
Note that the DG participants performed `Orienting' significantly more than those of CG ($t(42)=2.40$, $p=0.02$, $d=0.70$).  
To identify the correlation between the activities and the generated insights, we performed a correlation analysis following Guo et al.~\cite{Guo16}. 
The results are shown in Table~\ref{tab_correlation}. 
To report the strength of the correlation results, we use the interpretation guidelines proposed by Evans~\cite{Evans96}: $0.8 \leq r$ for very strong; $0.6 \leq r < 0.79$ for strong; and $0.4 \leq r<0.59$ for moderate.
We found that \textit{Comparing} had a very strong correlation with having observations ($r=0.87$, $p<0.001$), hypotheses ($r=0.88$, $p=0.01$), and questions ($r=0.96$, $p<0.001$), and \textit{Orienting} had a strong correlation with having observations ($r=0.66$, $p<0.001$), hypotheses ($r=0.8$, $p=0.03$), questions ($r$=0.67, $p<0.001$) and comments ($r=0.44$, $p=0.03$).
Furthermore, \textit{Narrowing} had a strong correlation with having observations ($r=0.68$, $p<0.001$) and comments ($r=0.63$, $p<0.001$).
Interestingly \tech{} itself had strong correlation with generation of the goal insights ($r=0.63$, $p<0.001$). %

Recommending interactions can further facilitate visual analysis~\cite{Wongsuphasawat15}; however, what should be the best recommendations during view creation or visual analysis are not clear.
This may be a reason why no systems provide recommendations for interaction or analysis paths~\cite{Behrisch18}. 
We think that our observations on interactions sequences can be considered as an initial data for designing recommendations on multidimensional data anlaysis.

